Study of type-B QPOs observed in black hole X-ray binary Swift J1728.9-3613

We report the detection of type-B quasi-periodic oscillation (QPO) of the black hole X-ray binary Swift J1728.9-3613 observed by NICER during the 2019 outburst. A type- B QPO was observed for the first two days and it disappeared as flux increased, but again appeared at $\sim$ 7.70 Hz when flux was dramatically decreased. The source was found in the soft-intermediate state during these observations. We further studied the energy dependence of the QPO. We found that QPO was observed only for a higher energy range implying that the origin of QPO is possibly due to the corona emitting higher energy photons by the inverse Compton process. The variation of spectral parameters can be explained with the disk truncation model. The fractional rms found to be monotonically increased with energy. The phase lag spectrum followed the U-shaped curve. The rms and phase lag spectrum are modelled and explained with the single-component comptonization model vkompthdk.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

